Self-Adjusting Stack Machines

Self-adjusting computation offers a language-based approach to writing programs that automatically respond to dynamically changing data. Recent work made significant progress in developing sound semantics and associated implementations of self-adjusting computation for high-level, functional languages. These techniques, however, do not address issues that arise for low-level languages, i.e., stack-based imperative languages that lack strong type systems and automatic memory management. In this paper, we describe techniques for self-adjusting computation which are suitable for low-level languages. Necessarily, we take a different approach than previous work: instead of starting with a high-level language with additional primitives to support self-adjusting computation, we start with a low-level intermediate language, whose semantics is given by a stack-based abstract machine. We prove that this semantics is sound: it always updates computations in a way that is consistent with full reevaluation. We give a compiler and runtime system for the intermediate language used by our abstract machine. We present an empirical evaluation that shows that our approach is efficient in practice, and performs favorably compared to prior proposals.

==> fig-exptrees-c-code.tex <==
\begin{figure}
\centering

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=\kill
\codeLineL{line:evalc::typedef}\> 
\kw{typedef} \kw{struct} node\_s* node\_t;
\\
\codeLineL{line:evalc::struct-node}\> 
\kw{struct} node\_s \{
\\
\codeLineL{line:evalc::enum-op}\>\> 
\kw{enum} \{ LEAF, BINOP \} tag;
\\
\codeLineL{line:evalc::union}\>\> 
\kw{union} \{ int leaf\_val;
\\
\codeLineL{line:evalc::struct-binop}\>\>
~~~~~~~~\kw{struct} \{ \kw{enum} \{ PLUS, MINUS \} op;
\\
\codeLineL{line:evalc::struct-binop}\>\>
~~~~~~~~~~~~~~~~node\_t left, right;
\\
\codeLineL{line:evalc::struct-binop::end}\>\>\>
~~~~~~~~~~~~\} binop;
\\
\codeLineL{line:evalc::union::end}\>\>
~~~~~~\} u;
\\
\codeLineL{line:evalc::struct-node::end}\>
\}
\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{Type declarations for expression trees in C.}
\label{fig:exptrees-c-types}
\end{minipage}
\\[2mm]

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
\codeLineL{evalc::line:evalc::def}\>\kw{int} eval (node\_t root) \{
\\  
\codeLineL{line:evalc::ifleaf}\>\>
\kw{if} (root->tag == LEAF) 
\\
\codeLineL{line:evalc::thenleaf}\>\>\>
\kw{return} root->u.leaf\_val;
\\
\codeLineL{line:evalc::ifleafelse}\>\>
\kw{else} \{
\\
\codeLineL{line:evalc::firsteval}\>\>\>
\kw{int} l = eval (root->u.binop.left);
\\
\codeLineL{line:evalc::secondeval}\>\>\>
\kw{int} r = eval (root->u.binop.right);
\\[1mm]
\codeLineL{line:evalc::ifplus}\>\>\>
\kw{if} (root->u.binop.op == PLUS) \kw{return} (l + r); 
\\
%
%
%
\codeLineL{line:evalc::elseminus}\>\>\>
\kw{else} \kw{return} (l - r);
\\
\codeLineL{line:evalc::ifleafelseend}\>\>
\}
\\
\codeLineL{line:evalc::evalbrace} \> \}
\end{codeListing}
}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-c-eval}
\end{minipage}
\end{figure} 


\begin{comment}
\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
%
%
\> \kw{typedef} \kw{enum} \{ NODE, LEAF\} kind\_t;
\\[1mm]
\> \kw{typedef} \kw{struct} \{ ~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\>\> kind\_t kind; 
\\
\>\> \kw{enum} \{ PLUS, MINUS \} op;
\\
\>\> \kw{struct} node\_t *left, *right;
\\
\>\} node\_t;
\\[1mm]
\>\kw{typedef} \kw{struct} \{ 
\\
\>\> kind\_t kind; 
\\
\>\> int num;
\\
\>\} leaf\_t;
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{Data type definitions for expression trees.}
\label{fig:exptrees-dt}
\end{minipage}
\\[2mm]

\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
\codeLineL{evalc::line:evalc::def}\>\kw{int} eval (\kw{struct} node\_t *root) \{
\\  
\codeLineL{line:evalc::ifleaf}\>\>
\kw{if} (t->kind == LEAF) \{ \kw{return} num; \}
\\
\codeLineL{line:evalc::ifleafelse}\>\>
\kw{else} \{
\\
\codeLineL{line:evalc::firsteval}\>\>\>
a = eval (t->left);
\\
\codeLineL{line:evalc::secondeval}\>\>\>
b = eval (t->right);
\\%[2mm]
\codeLineL{line:evalc::ifplus}\>\>\>
\kw{if} (t->op == PLUS) \{ \kw{return} (a + b); \}
\\
\codeLineL{line:evalc::ifminus}\>\>\>
\kw{else} \{ \kw{return} (a - b); \}
\\
\codeLineL{line:evalc::ifleafelseend}\>\>
\}
\\
\codeLineL{line:evalc::evalbrace} \> \}
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-c-eval}
\label{fig:exptrees-eval-c}
\end{minipage}
\end{figure} 
\end{comment}


==> fig-exptrees-example-only-traces.tex <==
\begin{figure}
%
\includegraphics[height=0.85in]{exptrees-trace-timed-before}

\medskip
\smallskip

\includegraphics[height=0.85in]{exptrees-trace-timed-after}
\nocaptionrule
\vspace*{-2mm}
\caption{Example execution traces of \ttt{eval}%
.}
\label{fig:exptrees-example-only-traces}


\end{figure}



==> fig-exptrees-example-traces.tex <==
\begin{figure}
\begin{minipage}[t]{1.2in}
\centering
%
\includegraphics[width=1.0in]{exptree-before}

\smallskip
\medskip

\includegraphics[width=1.1in]{exptree-after}

\vspace*{-2mm}

\nocaptionrule
\caption{Expressions.}
\label{fig:exptrees-example}
%
\end{minipage}
%
\begin{minipage}[t]{1.8in}
\centering
\includegraphics[width=2.2in]{exptrees-trace-before}

\medskip
\smallskip

\includegraphics[width=2.2in]{exptrees-trace-after}

\nocaptionrule
\vspace*{-2mm}
\caption{And their traces.}
\label{fig:exptrees-traces}

\end{minipage}

\end{figure}



==> fig-exptrees-example.tex <==
\begin{figure}
\centering
\includegraphics[height=1.5in]{exptree-before}
\quad\quad
\includegraphics[height=1.5in]{exptree-after}

\nocaptionrule
\vspace*{-2mm}
\caption{Example expression trees.}
\label{fig:exptrees-example}
\vspace*{-4mm}
\end{figure}



==> fig-exptrees-il-code-delta.tex <==
{
\newcommand{\offsettag}{TAG}
\newcommand{\offsetval}{VAL}
\newcommand{\offsetop}{OP}
\newcommand{\offsetleft}{LEFT}
\newcommand{\offsetright}{RIGHT}

%

%
%
%
%
%
%
\newcommand{\hlbgl}[1]{#1}
\newcommand{\hlbgd}[1]{#1}

%

\newcommand{\hlboxl}[1]{
  \colorbox[gray]{0.95}{#1}
}
\newcommand{\hlboxd}[1]{
  \colorbox[gray]{0.88}{#1}
}

%

\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\setlength{\fboxsep}{0pt}%
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:il:fun}\>eval (root) =
\\  
\codeLineL{line:il:eval::ktwo::memo}\>\>
\kw{memo} 
\\
\codeLineL{line:il:eval::ktwo::def}\>\>
\kw{let} 
\\

\hspace{-13pt}
\hlboxl{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:il::kone::def}\>\>\>
\hlbgl{\kw{fun} \kone(l) =}
\\

\codeLineL{line:il::kone::let}\>\>\>
\hlbgl{\kw{let}}
\\


\hspace{-13pt}
\hlboxd{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:il:eval::ktwo::fun}\>\>\>\>
\hlbgd{\kw{fun}~\ktwo(r) =}
\\
\codeLineL{line:il:eval::ktwo::readop}\>\>\>\>
\hlbgd{~~\kw{update}}
\\
\codeLineL{line:il:eval::ktwo::readop::body}\>\>\>\>\>\>
\lineref{eval::ktwo::readop}--\lineref{eval::ktwo::else}
\end{tabbing}
\end{minipage}
}
\\

\codeLineL{line:il:kone::in}\>\>\>
\hlbgl{\kw{in}}
\\
\codeLineL{line:il:kone::in}\>\>\>\>
\hlbgl{\kw{update} }
\\
\codeLineL{line:il:kone::in::body}\>\>\>\>\>
\lineref{kone::in::push}--\lineref{kone::eval}
\end{tabbing}
\end{minipage}
}

\\[2mm]
%
\codeLineL{line:il:eval::in}\>\>
\kw{in}
\\
\codeLineL{line:il:eval::update}\>\>\>
\kw{update}
\\
\codeLineL{line:il:eval::update::body}\>\>\>\>
\lineref{eval::readtag}--\lineref{eval::else::push::do::end}

\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in \IL with
  self-adjusting-computation keywords.}
\label{fig:exptrees-il-code-delta}
\end{minipage}
\end{figure} 
}


==> fig-exptrees-il-code-deprecated.tex <==
{
\newcommand{\offsettag}{OFFSET\_TAG}
\newcommand{\offsetval}{OFFSET\_VAL}
\newcommand{\offsetop}{OFFSET\_OP}
\newcommand{\offsetleft}{OFFSET\_LEFT}
\newcommand{\offsetright}{OFFSET\_RIGHT}


\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:fun}\>eval (root) =
\\  
\codeLineL{line:eval::ktwo::def}\>
\kw{let} 
\\
\codeLineL{line:kone::def}\>\>
\kw{fun} \kone(a) =
\\
\codeLineL{line:kone::let}\>\>
\kw{let}
\\
\codeLineL{line:eval::ktwo::fun}\>\>\>
\kw{fun} \ktwo(b) =
\\
\codeLineL{line:eval::ktwo::readop}\>\>\>\>
op $=$ \kw{read} (root, \offsetop)
\\
\codeLineL{line:eval::ktwo::ifop}\>\>\>\>
\kw{if} (op == PLUS) \{
\\
\codeLineL{line:eval::ktwo::add}\>\>\>\>\>
r $=$ a+b
\\
\codeLineL{line:eval::ktwo::if::pop}\>\>\>\>\>
pop r
\\
\codeLineL{line:eval::ktwo::if::end}\>\>\>\>
\}
\\
\codeLineL{line:eval::ktwo::else}\>\>\>\>
\kw{else} \{
\\
\codeLineL{line:eval::ktwo::else::minus}\>\>\>\>\>
r $=$ a-b
\\
\codeLineL{line:eval::ktwo::else::pop}\>\>\>\>\>
pop r
\\
\codeLineL{line:eval::ktwo::else::end}\>\>\>\>
\}
\\
\codeLineL{line:kone::in}\>\>
\kw{in}
\\
\codeLineL{line:kone::in::push}\>\>
\>\kw{push} \ktwo~\kw{do} \{
\\
\codeLineL{line:kone::in}\>\>\>\>
\kw{update} \{
\\
\codeLineL{line:kone::read}\>\>\>\>\>
right $=$ \kw{read} (root, \offsetright)
\\
\codeLineL{line:kone::eval}\>\>\>\>\>
eval right
\\
\codeLineL{line:kone::eval::update::end}\>\>\>\>
\}
\\
\codeLineL{line:kone::in::push::end}\>\>\>
\}
\\
\codeLineL{line:kone::end}\>\>
\kw{end}
\\[2mm]
%
\codeLineL{line:eval::in}\>
\kw{in}
\\
\codeLineL{line:eval::memo}\>\>
\kw{memo} \{
\\
\codeLineL{line:eval::readtag}\>\>\>
tag $=$ \kw{read} (root,\offsettag) \kw{in}
\\
\codeLineL{line:eval::iftag}\>\>\>
\kw{if} (tag == LEAF) \{
\\
\codeLineL{line:eval::iftagleaf}\>\>\>\>
num $\leftarrow$ \kw{read} (root,\offsetval)
\\
\codeLineL{line:eval::pop}\>\>\>\>
\kw{pop} num
\\
\codeLineL{line:eval::else}\>\>\>
\kw{else}
\\
\codeLineL{line:eval::else::push}\>\>\>\>
\kw{push} \kone~\kw{do}  \{
\\
\codeLineL{line:eval::else::push::do::update}\>\>\>\>\>
\kw{update} \{
\\
\codeLineL{line:eval::else::push::do::update::read}\>\>\>\>\>\>
left $=$ \kw{read} (root, \offsetleft)
\\
\codeLineL{line:eval::else::push::do::update::eval}\>\>\>\>\>\>
eval (left)
\\
\codeLineL{line:eval::in::update::end}\>\>\>\>\>
\}
\\
\codeLineL{line:eval::in::push}\>\>\>\>
\}
\\
\codeLineL{line:eval::memoEnd}\>\>\>
\}
\\
\codeLineL{line:eval::end}\>
\kw{end}
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-eval-il-code}
\end{minipage}
\end{figure} 
}


==> fig-exptrees-il-code-sugared.tex <==
{
\newcommand{\offsettag}{OFFSET\_TAG}
\newcommand{\offsetval}{OFFSET\_VAL}
\newcommand{\offsetop}{OFFSET\_OP}
\newcommand{\offsetleft}{OFFSET\_LEFT}
\newcommand{\offsetright}{OFFSET\_RIGHT}

%

%
%
%
%
%
%
\newcommand{\hlbgl}[1]{#1}
\newcommand{\hlbgd}[1]{#1}

%

\newcommand{\hlboxl}[1]{
\colorbox[gray]{0.90}{#1}
}
\newcommand{\hlboxd}[1]{
\colorbox[gray]{0.80}{#1}
}

%

\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\setlength{\fboxsep}{0pt}%
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:fun}\>eval (root) =
\\  
\codeLineL{line:eval::ktwo::def}\>
\kw{let} 
\\

\hspace{-13pt}
\hlboxl{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:kone::def}\>\>\>
\hlbgl{\kw{fun} \kone(a) =}
\\
\codeLineL{line:kone::let}\>\>\>
\hlbgl{\kw{let}}
\\

\hspace{-13pt}
\hlboxd{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:eval::ktwo::fun}\>\>\>\>
\hlbgd{\kw{fun} \ktwo(b) =}
\\
\codeLineL{line:eval::ktwo::readop}\>\>\>\>
\hlbgd{~~op $=$ \kw{read} (root, \offsetop)}
\\
\codeLineL{line:eval::ktwo::ifop}\>\>\>\>
\hlbgd{~~\kw{if} (op == PLUS) \{ pop (a+b) \}}
\\
\codeLineL{line:eval::ktwo::else}\>\>\>\>
\hlbgd{~~\kw{else} \{ pop (a-b) \}}

\end{tabbing}
\end{minipage}
}
\\

\codeLineL{line:kone::in}\>\>\>
\hlbgl{\kw{in}}
\\
\codeLineL{line:kone::in::push}\>\>\>
\hlbgl{~~\kw{push} \ktwo~\kw{do} \{}
\\
\codeLineL{line:kone::in}\>\>
\hlbgl{~~~~~~\kw{update} \{}
\\
\codeLineL{line:kone::read}\>\>
\hlbgl{~~~~~~~~right $=$ \kw{read} (root, \offsetright)}
\\
\codeLineL{line:kone::eval}\>\>
\hlbgl{~~~~~~~~eval (right)}
\\
\codeLineL{line:kone::eval::update::end}\>\>
\hlbgl{~~~~~~\}}
\\
\codeLineL{line:kone::in::push::end}\>\>
\hlbgl{~~~~\}}
\\
\codeLineL{line:kone::end}\>\>\>
\hlbgl{\kw{end}}

\end{tabbing}
\end{minipage}
}

\\[2mm]
%
\codeLineL{line:eval::in}\>
\kw{in}
\\
\codeLineL{line:eval::memo}\>\>
\kw{memo} \{
\\
\codeLineL{line:eval::readtag}\>\>\>
tag $=$ \kw{read} (root,\offsettag)
\\
\codeLineL{line:eval::iftag}\>\>\>
\kw{if} (tag == LEAF) \{
\\
\codeLineL{line:eval::iftagleaf}\>\>\>\>
num $=$ \kw{read} (root,\offsetval)
\\
\codeLineL{line:eval::pop}\>\>\>\>
\kw{pop} num
\\
\codeLineL{line:eval::iftagleaf::end}\>\>\>\>
\}
\\
\codeLineL{line:eval::else}\>\>\>
\kw{else} \{
\\
\codeLineL{line:eval::else::push}\>\>\>\>
\kw{push} \kone~\kw{do}  \{
\\
\codeLineL{line:eval::else::push::do::update}\>\>\>\>\>
\kw{update} \{
\\
\codeLineL{line:eval::else::push::do::update::read}\>\>\>\>\>\>
left $=$ \kw{read} (root, \offsetleft)
\\
\codeLineL{line:eval::else::push::do::update::eval}\>\>\>\>\>\>
eval (left)
\\
\codeLineL{line:eval::in::update::end}\>\>\>\>\>
\}
\\
\codeLineL{line:eval::in::push::end}\>\>\>\>
\}
\\
\codeLineL{line:eval::else::end}\>\>\>
\}
\\
\codeLineL{line:eval::memoEnd}\>\>
\}
\\
\codeLineL{line:eval::end}\>
\kw{end}
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-eval-il-code}
\end{minipage}
\end{figure} 
}


==> fig-exptrees-il-code.tex <==
{
\newcommand{\offsettag}{TAG}
\newcommand{\offsetval}{LEAF\_VAL}
\newcommand{\offsetop}{OP}
\newcommand{\offsetleft}{LEFT}
\newcommand{\offsetright}{RIGHT}

%

%
%
%
%
%
%
\newcommand{\hlbgl}[1]{#1}
\newcommand{\hlbgd}[1]{#1}

%

\newcommand{\hlboxl}[1]{
  \colorbox[gray]{0.95}{#1}
}
\newcommand{\hlboxd}[1]{
  \colorbox[gray]{0.88}{#1}
}

%

\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\setlength{\fboxsep}{0pt}%
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:il:fun}\>eval (root) =
\\  
\codeLineL{line:il:eval::ktwo::def}\>
\kw{let} 
\\

\hspace{-13pt}
\hlboxl{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:il:kone::def}\>\>\>
\hlbgl{\kw{fun} \kone(l) =}
\\
\codeLineL{line:il:kone::let}\>\>\>
\hlbgl{\kw{let}}
\\

\hspace{-13pt}
\hlboxd{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:il:eval::ktwo::fun}\>\>\>\>
\hlbgd{\kw{fun}~\ktwo(r) =}
\\
\codeLineL{line:il:eval::ktwo::readop}\>\>\>\>
\hlbgd{~~\kw{update}}
\\
\codeLineL{line:il:eval::ktwo::readop}\>\>\>\>\>
\hlbgd{~~\kw{let}~op $=$ \kw{read} (root[\offsetop])}~\kw{in}
\\
\codeLineL{line:il:eval::ktwo::ifop}\>\>\>\>\>\>
\hlbgd{~~\kw{if} (op == PLUS)  \kw{pop} (l+r)}
\\
\codeLineL{line:il:eval::ktwo::else}\>\>\>\>\>\>
\hlbgd{~~\kw{else} \kw{pop} (l-r) }

\end{tabbing}
\end{minipage}
}
\\

\codeLineL{line:il:kone::in}\>\>\>
\hlbgl{\kw{in}}
\\
\codeLineL{line:il:kone::in}\>\>\>\>
\hlbgl{\kw{update} }
\\
\codeLineL{line:il:kone::in::push}\>\>\>\>\>
\hlbgl{\kw{push} \ktwo~\kw{do}}
\\
\codeLineL{line:il:kone::read}\>\>\>\>\>
\hlbgl{\kw{let}~right $=$ \kw{read} (root[\offsetright])~\kw{in}}
\\
\codeLineL{line:il:kone::eval}\>\>\>\>\>\>
\hlbgl{eval (right)}
\end{tabbing}
\end{minipage}
}

\\[2mm]
%
\codeLineL{line:il:eval::in}\>
\kw{in}
\\
\codeLineL{line:il:eval::memo}\>\>
\kw{memo}
\\
\codeLineL{line:il:eval::update}\>\>\>
\kw{update}
\\
\codeLineL{line:il:eval::readtag}\>\>\>\>
\kw{let}~tag $=$ \kw{read} (root[\offsettag])~\kw{in}
\\
\codeLineL{line:il:eval::iftag}\>\>\>\>\>
\kw{if} (tag == LEAF) 
\\
\codeLineL{line:il:eval::iftagleaf}\>\>\>\>\>\>
\kw{let}~num $=$ \kw{read} (root[\offsetval])~\kw{in}
\\
\codeLineL{line:il:eval::pop}\>\>\>\>\>\>\>
\kw{pop} num
\\
\codeLineL{line:il:eval::else}\>\>\>\>\>
\kw{else} 
\\
\codeLineL{line:il:eval::else::push}\>\>\>\>\>\>
\kw{push} \kone~\kw{do}  
\\
\codeLineL{line:il:eval::else::push::do::read}\>\>\>\>\>\>\>
\kw{let}~left $=$ \kw{read} (root[\offsetleft])~\kw{in}
\\
\codeLineL{line:il:eval::else::push::do::end}\>\>\>\>\>\>\>\>
eval (left)
\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in \IL.}
\label{fig:exptrees-il-code}
\end{minipage}
\end{figure} 
}


==> fig-exptrees-il-static-code.tex <==
\begin{figure}
\centering

{
\newcommand{\offsettag}{TAG}
\newcommand{\offsetval}{VAL}
\newcommand{\offsetop}{OP}
\newcommand{\offsetleft}{LEFT}
\newcommand{\offsetright}{RIGHT}

%

%
%
%
%
%
%
\newcommand{\hlbgl}[1]{#1}
\newcommand{\hlbgd}[1]{#1}

%

\newcommand{\hlboxl}[1]{
  \colorbox[gray]{0.95}{#1}
}
\newcommand{\hlboxd}[1]{
  \colorbox[gray]{0.88}{#1}
}

%

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\setlength{\fboxsep}{0pt}%
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:fun}\>eval (root) =
\\  
\codeLineL{line:eval::ktwo::def}\>
\kw{let} 
\\

\hspace{-13pt}
\hlboxl{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:kone::def}\>\>\>
\hlbgl{\kw{fun} \kone(l) =}
\\
\codeLineL{line:kone::let}\>\>\>
\hlbgl{\kw{let}}
\\

\hspace{-13pt}
\hlboxd{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:eval::ktwo::fun}\>\>\>\>
\hlbgd{\kw{fun}~\ktwo(r) =}
\\
\codeLineL{line:eval::ktwo::readop}\>\>\>\>
\hlbgd{~~\kw{let}~op $=$ \kw{read} (root[\offsetop])}~\kw{in}
\\
\codeLineL{line:eval::ktwo::ifop}\>\>\>\>\>
\hlbgd{~~\kw{if} (op == PLUS)  \kw{pop} (l+r)}
\\
\codeLineL{line:eval::ktwo::else}\>\>\>\>\>
\hlbgd{~~\kw{else} \kw{pop} (l-r) }

\end{tabbing}
\end{minipage}
}
\\

\codeLineL{line:kone::in}\>\>\>
\hlbgl{\kw{in}}
\\
\codeLineL{line:kone::in::push}\>\>\>\>
\hlbgl{\kw{push} \ktwo \kw{do}}
\\
%
%
%
\codeLineL{line:kone::read}\>\>\>\>\>
\hlbgl{\kw{let}~right $=$ \kw{read} (root[\offsetright])~\kw{in}}
\\
\codeLineL{line:kone::eval}\>\>\>\>\>\>
\hlbgl{eval (right)}
\end{tabbing}
\end{minipage}
}

\\[2mm]
%
\codeLineL{line:eval::in}\>
\kw{in}
\\
%
%
%
%
%
%
\codeLineL{line:eval::readtag}\>\>
\kw{let}~tag $=$ \kw{read} (root[\offsettag])~\kw{in}
\\
\codeLineL{line:eval::iftag}\>\>\>
\kw{if} (tag == LEAF) 
\\
\codeLineL{line:eval::iftagleaf}\>\>\>\>
\kw{let}~val $=$ \kw{read} (root[\offsetval])~\kw{in}
\\
\codeLineL{line:eval::pop}\>\>\>\>\>
\kw{pop} val
\\
\codeLineL{line:eval::else}\>\>\>
\kw{else} 
\\
\codeLineL{line:eval::else::push}\>\>\>\>
\kw{push} \kone~\kw{do}  
\\
\codeLineL{line:eval::else::push::do::read}\>\>\>\>\>
\kw{let}~left $=$ \kw{read} (root[\offsetleft])~\kw{in}
\\
\codeLineL{line:eval::else::push::do::end}\>\>\>\>\>\>
eval (left)
\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in \IL.}
%
\label{fig:exptrees-il-static-code}
\end{minipage}
}

\end{figure} 




==> fig-exptrees-traces.tex <==
\begin{figure}
\centering
\includegraphics[width=3.0in]{exptrees-trace-before}

\medskip
\smallskip

\includegraphics[width=3.0in]{exptrees-trace-after}

\nocaptionrule
%
\caption{Traces for executions of \ttt{eval}
  (\figref{exptrees-eval-il-static-code}) with the trees in
  \figref{exptrees-example}.  The top and bottom traces each
  corresponds to the left and the right tree of
  \figref{exptrees-example} respectively.
}
\label{fig:exptrees-traces}
\vspace*{-4mm}
\end{figure}



==> fig-exptrees.tex <==
%
%
%
%
%
%

\begin{figure}
\centering

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=\kill
\codeLineL{line:evalc::typedef}\> 
\kw{typedef} \kw{struct} node\_s* node\_t;
\\
\codeLineL{line:evalc::struct-node}\> 
\kw{struct} node\_s \{
\\
\codeLineL{line:evalc::enum-op}\>\> 
\kw{enum} \{ LEAF, BINOP \} tag;
\\
\codeLineL{line:evalc::union}\>\> 
\kw{union} \{ int leaf;
\\
\codeLineL{line:evalc::struct-binop}\>\>
~~~~~~~~\kw{struct} \{ \kw{enum} \{ PLUS, MINUS \} op;
\\
\codeLineL{line:evalc::struct-binop}\>\>
~~~~~~~~~~~~~~~~node\_t left, right;
\\
\codeLineL{line:evalc::struct-binop::end}\>\>\>
~~~~~~~~~~~~\} binop;
\\
\codeLineL{line:evalc::union::end}\>\>
~~~~~~\} u;
\\
\codeLineL{line:evalc::struct-node::end}\>
\}
\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{Type declarations for expression trees in C.}
\label{fig:exptrees-c-types}
\end{minipage}
\\[2mm]

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
\codeLineL{evalc::line:evalc::def}\>\kw{int} eval (node\_t root) \{
\\  
\codeLineL{line:evalc::ifleaf}\>\>
\kw{if} (root->tag == LEAF) 
\\
\codeLineL{line:evalc::thenleaf}\>\>\>
\kw{return} root->u.leaf;
\\
\codeLineL{line:evalc::ifleafelse}\>\>
\kw{else} \{
\\
\codeLineL{line:evalc::firsteval}\>\>\>
\kw{int} l = eval (root->u.binop.left);
\\
\codeLineL{line:evalc::secondeval}\>\>\>
\kw{int} r = eval (root->u.binop.right);
\\[1mm]
\codeLineL{line:evalc::ifplus}\>\>\>
\kw{if} (root->u.binop.op == PLUS) \kw{return} (l + r); 
\\
%
%
%
\codeLineL{line:evalc::elseminus}\>\>\>
\kw{else} \kw{return} (l - r);
\\
\codeLineL{line:evalc::ifleafelseend}\>\>
\}
\\
\codeLineL{line:evalc::evalbrace} \> \}
\end{codeListing}
}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-c-eval}
\end{minipage}
\\[2mm]

{
\newcommand{\offsettag}{TAG}
\newcommand{\offsetval}{VAL}
\newcommand{\offsetop}{OP}
\newcommand{\offsetleft}{LEFT}
\newcommand{\offsetright}{RIGHT}

%

%
%
%
%
%
%
\newcommand{\hlbgl}[1]{#1}
\newcommand{\hlbgd}[1]{#1}

%

\newcommand{\hlboxl}[1]{
  \colorbox[gray]{0.95}{#1}
}
\newcommand{\hlboxd}[1]{
  \colorbox[gray]{0.88}{#1}
}

%

\begin{minipage}{\columnwidth}
\fixedCodeFrame{\parbox{0.8\columnwidth}{
\setlength{\fboxsep}{0pt}%
\begin{codeListing}
XXXX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill
\codeLineL{line:fun}\>eval (root) =
\\  
\codeLineL{line:eval::ktwo::def}\>
\kw{let} 
\\

\hspace{-13pt}
\hlboxl{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:kone::def}\>\>\>
\hlbgl{\kw{fun} \kone(l) =}
\\
\codeLineL{line:kone::let}\>\>\>
\hlbgl{\kw{let}}
\\

\hspace{-13pt}
\hlboxd{
\begin{minipage}{\columnwidth}
\begin{tabbing}
XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=XX\=
\kill

\codeLineL{line:eval::ktwo::fun}\>\>\>\>
\hlbgd{\kw{fun}~\ktwo(r) =}
\\
\codeLineL{line:eval::ktwo::readop}\>\>\>\>
\hlbgd{~~\kw{update}}
\\
\codeLineL{line:eval::ktwo::readop}\>\>\>\>\>
\hlbgd{~~\kw{let}~op $=$ \kw{read} (root[\offsetop])}~\kw{in}
\\
\codeLineL{line:eval::ktwo::ifop}\>\>\>\>\>\>
\hlbgd{~~\kw{if} (op == PLUS)  \kw{pop} (l+r)}
\\
\codeLineL{line:eval::ktwo::else}\>\>\>\>\>\>
\hlbgd{~~\kw{else} \kw{pop} (l-r) }

\end{tabbing}
\end{minipage}
}
\\

\codeLineL{line:kone::in}\>\>\>
\hlbgl{\kw{in}}
\\
\codeLineL{line:kone::in::push}\>\>\>\>
\hlbgl{\kw{push} \ktwo \kw{do}}
\\
\codeLineL{line:kone::in}\>\>\>\>\>
\hlbgl{\kw{update} }
\\
\codeLineL{line:kone::read}\>\>\>\>\>\>
\hlbgl{\kw{let}~right $=$ \kw{read} (root[\offsetright])~\kw{in}}
\\
\codeLineL{line:kone::eval}\>\>\>\>\>\>\>
\hlbgl{eval (right)}
\end{tabbing}
\end{minipage}
}

\\[2mm]
%
\codeLineL{line:eval::in}\>
\kw{in}
\\
\codeLineL{line:eval::memo}\>\>
\kw{memo}
\\
\codeLineL{line:eval::update}\>\>\>
\kw{update}
\\
\codeLineL{line:eval::readtag}\>\>\>\>
\kw{let}~tag $=$ \kw{read} (root[\offsettag])~\kw{in}
\\
\codeLineL{line:eval::iftag}\>\>\>\>\>
\kw{if} (tag == LEAF) 
\\
\codeLineL{line:eval::iftagleaf}\>\>\>\>\>\>
\kw{let}~val $=$ \kw{read} (root[\offsetval])~\kw{in}
\\
\codeLineL{line:eval::pop}\>\>\>\>\>\>\>
\kw{pop} val
\\
\codeLineL{line:eval::else}\>\>\>\>\>
\kw{else} 
\\
\codeLineL{line:eval::else::push}\>\>\>\>\>\>
\kw{push} \kone~\kw{do}  
\\
\codeLineL{line:eval::else::push::do::read}\>\>\>\>\>\>\>
\kw{let}~left $=$ \kw{read} (root[\offsetleft])~\kw{in}
\\
\codeLineL{line:eval::else::push::do::end}\>\>\>\>\>\>\>\>
eval (left)
\end{codeListing}}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in \IL.}
\label{fig:exptrees-il-code}
\label{fig:exptrees-il-eval}
\label{fig:exptrees-eval-il-code}
\end{minipage}
}

\end{figure} 


\begin{comment}
\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
%
%
\> \kw{typedef} \kw{enum} \{ NODE, LEAF\} kind\_t;
\\[1mm]
\> \kw{typedef} \kw{struct} \{ ~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\>\> kind\_t kind; 
\\
\>\> \kw{enum} \{ PLUS, MINUS \} op;
\\
\>\> \kw{struct} node\_t *left, *right;
\\
\>\} node\_t;
\\[1mm]
\>\kw{typedef} \kw{struct} \{ 
\\
\>\> kind\_t kind; 
\\
\>\> int num;
\\
\>\} leaf\_t;
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{Data type definitions for expression trees.}
\label{fig:exptrees-dt}
\end{minipage}
\\[2mm]

\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing}
XXXX\=XX\=XX\=XX\=\kill
\codeLineL{evalc::line:evalc::def}\>\kw{int} eval (\kw{struct} node\_t *root) \{
\\  
\codeLineL{line:evalc::ifleaf}\>\>
\kw{if} (t->kind == LEAF) \{ \kw{return} num; \}
\\
\codeLineL{line:evalc::ifleafelse}\>\>
\kw{else} \{
\\
\codeLineL{line:evalc::firsteval}\>\>\>
a = eval (t->left);
\\
\codeLineL{line:evalc::secondeval}\>\>\>
b = eval (t->right);
\\%[2mm]
\codeLineL{line:evalc::ifplus}\>\>\>
\kw{if} (t->op == PLUS) \{ \kw{return} (a + b); \}
\\
\codeLineL{line:evalc::ifminus}\>\>\>
\kw{else} \{ \kw{return} (a - b); \}
\\
\codeLineL{line:evalc::ifleafelseend}\>\>
\}
\\
\codeLineL{line:evalc::evalbrace} \> \}
\end{codeListing}}
\nocaptionrule
\vspace*{-2mm}
\caption{The \ttt{eval} function in C.}
\label{fig:exptrees-c-eval}
\label{fig:exptrees-eval-c}
\end{minipage}
\end{figure} 
\end{comment}


==> fig-il-tracing-rewind.tex <==
\begin{figure}
\[
\begin{array}{lcl}
{\trz{\trcons{\Pi}{t}}{T}} ; {T'}
& \trrewind &
{\trz{\Pi}{T}} ; \trcons{t}{T'}
\\
{\trz{\trcons{\Pi}{\trxundomark{T_2}}}{T_1}} ; T'
& \trrewind &
{\trz{\Pi}{\trcons{\trpush{T_1}}{T_2}}} ; T'
\end{array}
\]
\mycaptionrule
\caption{Rewinding the trace ($\circlearrowleft$).}
\end{figure}


==> fig-il-tracing-steps-eval.tex <==
\inferrule*[right=\refevalu]
{
\ilustate
{\sigma}
{\kappa}
{\rho}
{\iluexp}
%
\ilusteprel
%
\ilustate
{\sigma}
{\kappa}
{\rho'}
{e}
}%
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\iluexp}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho'}
{e}
}

\inferrule*[right=\refevalalloc]
{
\storestin{\sigma}{\rho}{\ilalloc{y}} 
\storestep 
\storestout{\sigma'}{\ell}
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\illet{\ilvar{x}{\ilalloc{y}}}{e}}
%
\iltevalstep
%
\iltstate
{\sigma'}
{\trz{\trcons{\trx}{\tralloc{\ell}{\rho(y)}}}{T}}
{\kappa}
{\rho[x\mapsto \ell]}
{e}
}

\inferrule*[right=\refevalread]
{
\storestin{\sigma}{\rho}{\ilread{y}{z}} \storestep \storestout{\sigma}{\nu}
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\illet{\ilvar{x}{\ilread{y}{z}}}{e}}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trread{\nu}{\rho(y)}{\rho(z)}}}{T}}
{\kappa}
{\rho[x \mapsto \nu]}
{e}
}

\inferrule*[right=\refevalwrite]
{
\storestin{\sigma}{\rho}{\ilwrite{x}{y}{z}} \storestep \storestout{\sigma'}{0}
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\illet{\ilvar{\_}{\ilwrite{x}{y}{z}}}{e}}
%
\iltevalstep
%
\iltstate
{\sigma'}
{\trz{\trcons{\trx}{\trwrite{\rho(z)}{\rho(x)}{\rho(y)}}}{T}}
{\kappa}
{\rho}
{e}
}

\inferrule*[right=\refevalmemo]
{
\strut
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\ilmemo{e}}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trmemo{\rho}{e}}}{T}}
{\kappa}
{\rho}
{e}
}

\inferrule*[right=\refevalwake]
{
\strut
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\ilwake{e}}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trwake{\rho}{e}}}{T}}
{\kappa}
{\rho}
{e}
}

\inferrule*[right=\refevalpush]
{
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\ilpush{f}{e}}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trxpushmark}}{T}}
%
{\stcons{\kappa}{\mkstframe{\rho}{f}}}
{\rho}
{e}
}

\inferrule*[right=\refevalpop]
{
  \vec \nu = \rho\fromto{(x_i)}{i=1}{|\vec x|}  
}
{
\iltstate
{\sigma}
{\trz{\trx}{T}}
{\kappa}
{\rho}
{\ilpop {\vec x}}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trpop{\vec \nu}}}{T}}
{\kappa}
{\emptyenv}
{\vec \nu}
}

\inferrule*[right=\refevalv]
{\trz{\trx}{T_2} ; \trend
  \trrewind^\ast
  \trz{\trcons{\trx'}{\trxpushmark}}{T'_2}; T_1 
  %
  \\
  \rho(f) = \ilfun{f}{\vec x}{e}
  \\
  \rho' = \rho\fromto{[x_i \mapsto \nu_i]}{i=1}{|\vec x|}
}
{
\iltstate
{\sigma}
{\trz{\trx}{T_2}}
{\stcons{\kappa}{\mkstframe{\rho}{f}}}
{\emptyenv}
{\vec \nu}
%
\iltevalstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx'}{\trpush{T_1}}}{T'_2}}
{\kappa}
{\rho'}
{e}
}


==> fig-il-tracing-steps-prop.tex <==
\inferrule*[right=\refpropalloc]
{
\storestin{\sigma}{\emptyenv}{\ilalloc{n}} \storestep \storestout{\sigma'}{\ell}
}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\tralloc{\ell}{n}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma'}
{\trz{\trcons{\trx}{\tralloc{\ell}{n}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refpropread]
{
\storestin{\sigma}{\emptyenv}{\ilread{\ell}{n}} \storestep \storestout{\sigma}{\nu}
}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trread{\nu}{\ell}{n}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trread{\nu}{\ell}{n}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refpropwrite]
{
\storestin{\sigma}{\emptyenv}{\ilwrite{\ell}{n}{\nu}} \storestep \storestout{\sigma'}{0}
}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trwrite{\nu}{\ell}{n}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma'}
{\trz{\trxcons{\trx}{\trwrite{\nu}{\ell}{n}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refpropmemo]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trmemo{\rho}{e}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trmemo{\rho}{e}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refpropwake]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trwake{\rho}{e}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trwake{\rho}{e}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refproppush]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trpush{T_1}}{T_2}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trxpropmark{T_2}}}{T_1}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right=\refproppop]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trpop{\vec \nu}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trpop{\vec \nu}}}{\trend}}
{\kappa}
{\emptyenv}
{\vec \nu}
}

\inferrule*[right=\refpropv]
{
\trz{\trx}{\trend}; \trend
\trrewind^\ast
\trz{\trcons{\trx'}{\trxpropmark{T_2}}}{\trend}; T_1
}
{
\iltstate
{\sigma}
{\trz{\trx}{\trend}}
{\kappa}
{\emptyenv}
{\vec \nu}
%
\iltpropstep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx'}{\trpush{T_1}}}{T_2}}
{\kappa}
{\emptyenv}
{\ilprop}
}



==> fig-il-tracing-steps-undo.tex <==
\inferrule*[right=\refundoalloc]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\tralloc{\ell}{n}}{\tr}}}
{\kappa}
{\rho}
{\rcmd}
%
\iltundostep
%
\iltstate
{\sigma[\ell \mapsto \storegarb]}
{\trz{\trx}{\tr}}
{\kappa}
{\rho}
{\rcmd}
} 

\inferrule*[right=\refundostep]
{
(t=\trread{\_}{\_}{\_}~
  |~\trwrite{\_}{\_}{\_}~
  |~\trmemo{\_}{\_}~
  |~\trwake{\_}{\_}~
  |~\trpop{\vec \nu}
)
}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{t}{\tr}}}
{\kappa}
{\rho}
{\rcmd}
%
\iltundostep
%
\iltstate
{\sigma}
{\trz{\trx}{\tr}}
{\kappa}
{\rho}
{\rcmd}
}

\inferrule*[right=\refundopush]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trpush{\tr_1}}{\tr_2}}}
{\kappa}
{\rho}
{\rcmd}
%
\iltundostep
%
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trxundomark{\tr_2}}}{\tr_1}}
{\kappa}
{\rho}
{\rcmd}
}

\inferrule*[right=\refundomark]
{\strut}
{
\iltstate
{\sigma}
{\trz{\trcons{\trx}{\trxundomark{\tr}}}{\trend}}
{\kappa}
{\rho}
{\rcmd}
%
\iltundostep
%
\iltstate
{\sigma}
{\trz{\trx}{\tr}}
{\kappa}
{\rho}
{\rcmd}
}


==> fig-il-tracing-steps.tex <==
\newcommand{\rulerule}{
\vspace{1mm}
\rule{0.90\textwidth}{1.5pt}
\and
\vspace{1mm}
}
\begin{figure*}
\centering
\begin{minipage}{\textwidth}
\begin{mathpar}
\noindent
\input{fig-il-tracing-steps-eval}
\and
\rulerule
%
\inferrule*[right={\bf E.P}]
{ }
{
\iltstate
{\sigma}
{\trz{\trx}{\trcons{\trmemo{\rho}{e}}{T}}}
{\kappa}
{\rho}
{\ilmemo{e}}
%
\iltevalpropstep
%
\iltstate
{\sigma}
{\trz{\trxcons{\trx}{\trmemo{\rho}{e}}}{T}}
{\kappa}
{\emptyenv}
{\ilprop}
}

\inferrule*[right={\bf P.E}]
{ }
{
\iltstate
{\sigma}
{\trz{\Pi}{\trcons{\trwake{\rho}{e}}{T}}}
{\kappa}
{\emptyenv}
{\ilprop}
%
\iltpropevalstep
%
\iltstate
{\sigma}
{\trz{\trxcons{\Pi}{\trwake{\rho}{e}}}{T}}
{\kappa}
{\rho}
{e}
}
\and
%
\rulerule
\input{fig-il-tracing-steps-prop}
\rulerule
%
\input{fig-il-tracing-steps-undo}
\end{mathpar}
\caption{Stepping relation for tracing machine ($\iltsteprel$).}
\label{fig:il-tracing-steps}
\end{minipage}
%

%
%
%
%
%
%
\end{figure*}


==> fig-il-tracing-subtrace-focusing.tex <==
\begin{figure}
%
%
%
\includegraphics[width=\columnwidth,page=3]
{ipe-trace-transformations}
\caption{Evaluating, undoing and propagating under subtraces.}
\label{fig:il-tracing-subtrace-focusing}
\end{figure}


==> fig-sparsemat-c-code.tex <==
\begin{figure}
\centering
\begin{minipage}{\columnwidth}
\fixedCodeFrame{
\begin{codeListing8}
X\=XX\=XX\=XX\=\kill
%
%

%
%
%
%
%

\> typedef struct svec\_s* svec\_t;
\\
\> struct svec\_s \{ long ix; data\_t val; svec\_t next; \};
\\
\> typedef struct smat\_s* smat\_t;
\\
\> struct smat\_s \{ long rowc; long colc; svec\_t* rowv; \};
\\

%
\\[2mm]
%

\> smat\_t smat\_transpose(smat\_t a) \{
\\
\>\> smat\_t b = alloc(struct smat\_s);
\\
\>\> b->colc = a->rowc; b->rowc = a->colc;
\\
\>\> b->rowv = alloc(svec\_t[b->rowc]);

\\%[1mm]

\>\> for(long i = 0; i < a->rowc; i++) \{
\\
\>\>\> svec\_t v = a->rowv[i];
\\
\>\>\> while(v) \{ svec\_t w = svec\_cons(i, v->val);
\\
\>\>\>\>~~~~~~~~~long j = v->ix; w->next = b->rowv[j];
\\
\>\>\>\>~~~~~~~~~b->rowv[j] = w; v = v->next; \}
\\
%
\>\> \}

\\%[1mm]

\>\> for(long j = 0; j < b->rowc; j++) 
\\
\>\>\>  b->rowv[j] = svec\_reverse(b->rowv[j]);

\\%[1mm]

\>\>  return b;
\\
\> \}

%
\\[2mm]
%

\> svec\_t smat\_svec\_mult(smat\_t m, svec\_t v) \{
\\
\>\> svec\_t* w = NULL;

\\%[1mm]

\>\> for(long i = 0; i < m->rowc; i++) \{
\\
\>\>\> data\_t d = svec\_dot(m->rowv[i], v);
\\      
\>\>\> if(nonzero(d)) \{ svec\_t w\_new = svec\_cons(i, d);
\\
\>\>\>\>~~~~~~~~~~~~~~ w\_new->next = w; w = w\_new; \}
\\
\>\> \}

\\%[2mm]

\>\> return svec\_reverse(w);
\\
\> \}

%
\\[2mm]
%

\> smat\_t smat\_smat\_mult(smat\_t a, smat\_t b) \{
\\

\>\> smat\_t c = smat\_transpose(b);

\\%[1mm]

\>\> for(long i = 0; i < c->rowc; i++)
\\
\>\>\> c->rowv[i] = smat\_vec\_mult(a, c->rowv[i]);

\\%[1mm]

\>\>  return smat\_transpose(c);
\\
\> \}
%
\end{codeListing8}}
\end{minipage}
\nocaptionrule
\vspace*{-2mm}
\caption{Sparse vectors and sparse matrices in \SRCC.}
\label{fig:sparsemat-c-code}
\end{figure}


==> fig-transpose.tex <==
\begin{figure}
\begin{codeListing}
XX\=XX\=XX\=XX\=XX\=\kill

mat\_t transpose(mat\_t m\_in) \{
\\
\>
mat\_t m\_out = mat\_skel(m\_in->n\_col, m\_in->n\_row);    
\\
\>
for (long i = 0; i < m\_in->n\_row; i++) \{
\\
\>\>
vec\_t v\_in = m\_in->row[i];
\\      
\>\>
while(v\_in) \{      
\\
\>\>\>
vec\_t w = vec\_cons(i, v\_in->value);
\\
%
%
%
\>\>\>
long j = v\_in->index;
\\        
\>\>\>
/* Push w onto the jth output row. */
\\
\>\>\>
w->next = m\_out->row[j];
\\
\>\>\>
m\_out->row[j] = w;
\\        
\>\>\>
v\_in = v\_in->next;
\\
\>\>\}
\\
\>
\}
\\  
\>
\\
\>
/* Reverse each new row. */
\>
\\
\>for (long j = 0; j < m\_out->n\_row; j++) \{
\\
%
%
\>\>
m\_out->row[j] = vec\_reverse(m\_out->row[j]);
%
%
\\
\>\}
\>
\\  
\>
return m\_out;
\\
\}
\end{codeListing}

\caption{Pseudo code for sparse matrix transpose in \SRCC.}
\end{figure}


==> iltraced-lemmas.tex <==
\subsection{Miscellaneous properties}

\TODO This section is temporary---it contains some lemmas that may be
useful (and may end up in a technical report, perhaps). Some of them
may not actually be useful to prove anything else.

\paragraph{Rewinding short hand} The following short hand make some
uses of trace rewinding more concise:
\[
\begin{array}{ccccc}
%
%
%
%
  {\Pi'} \trrewind \Pi
  &\equiv& 
  \trzip {\Pi'} \_ ; \_ \trrewind \trzip \Pi \_ ; \_
\end{array}
\]

\begin{lem}[Trace paths witness ``stack parametricity'' properties]~
\begin{enumerate}
%
\item
If~$\iltstatec
\_ {\trzip \Pi \_} \kappa \_ 
\iltsteprel^\ast
\iltstatec
\_ {\trzip {\Pi'} \_} {\kappa'} \_ 
$
\\
and~$\Pi' \trrewind^\ast \Pi$
\\
implies $\kappa = \kappa'$


\item
~$\iltstatec
\sigma {\trzip \Pi \trend} \_ \closedaction
\iltsteprel^\ast
\iltstatec
{\sigma'} {\trzip {\Pi'} \trend} \_ {\closedaction'}$
\\
and~$\Pi' \trrewind^\ast \Pi$
\\
if and only if
\\
$\ilustatec
\sigma \cdot \closedaction
\ilusteprel^\ast
\ilustatec
{\sigma'} \cdot {\closedaction'}
$

\item
If $\iltstatec
\sigma {\trzip \Pi \trend} \_ \closedaction
\iltsteprel^\ast
\iltstatec
{\sigma'} {\trzip {\Pi'} \trend} \_ {\closedaction'}
$
\\
and~$\Pi' \trrewind^\ast \Pi$
\\
then~$\iltstatec
\sigma {\trzip \Pi \trend} \cdot \closedaction
\iltsteprel^\ast
\iltstatec
{\sigma'} {\trzip {\Pi'} \trend} \cdot {\closedaction'}$
\\
(Note that the converse does not hold---undo-resume elimination breaks
it).

\end{enumerate}

\end{lem}

%

\begin{lem}[Trace steps imply eval steps---assuming no reuse]~
\\
If 
$\iltbigstep 
\trend \sigma \closedaction
{\hlm{t} \cons \_} {\sigma''} {\vec \nu}
$
%
%
%
%
%
%
%
%
%
%
%
%
then
\begin{description}

\item[$t \ne \trstep{Push}{\_} \Longrightarrow$]~
\\
$\iltstatec \sigma {\trzip \Pi \trend} \kappa \closedaction$
\\
\hl{
  $
  \iltsteprel
  \iltstatec
  {\sigma'} {\trzip {\Pi \cons t} \trend} {\kappa} {\closedaction'}
  $
}
\\
$\iltsteprel^\ast \iltstatec
{\sigma''} {\trzip {\Pi''} \trend} {\kappa} {\vec \nu}$

\item[$t = \trstep{Push}{T} \Longrightarrow$]~
\\
$\iltstate \sigma {\trzip \Pi \trend} \kappa \rho {\ilpush l e}$
\\
\hl{
  $
  \iltsteprel
  \iltstate
  {\sigma} {\trzip {\trpresume \Pi} \trend} 
  {\kappa \cons \angpair l \rho} \rho e
  $
}
\\
\hl{
  $
  \iltsteprel^\ast
  \iltstate 
  {\sigma'} {\trzip {\Pi'} \trend} 
  {\kappa \cons \angpair l \rho} {\cdot} {\vec \nu}
  $
}
\\
\parbox[t]{0.1\textwidth}{~}~\parbox[t]{0.5 \textwidth}{
with
$
\trzip {\Pi'} \trend ; \trend
\trrewind^\ast
\trzip {\trpresume \Pi} \trend ; T
$
\\
and
$\rho(l) = \kw{block}~l(\vec x).e_l$
}
\\
\hl{
  $
  \iltsteprel \iltstate 
  {\sigma'} {\trzip {\Pi \cons \trstep{Push}{T}} \trend} \kappa 
  {\rho[\vec x \mapsto \vec \nu]} {e_l}
  $
}
\\
$\iltsteprel^\ast \iltstatec
{\sigma''} {\trzip {\Pi''} \trend} {\kappa} {\vec \nu}$



\end{description}
\end{lem}



==> space-tricks.tex <==
%
\setlength{\floatsep}{4mm}
%
\setlength{\textfloatsep}{4mm}
%
\setlength{\intextsep}{0mm}
%
\setlength{\abovecaptionskip}{0mm}
%
\setlength{\belowcaptionskip}{0mm}

%
\renewcommand{\topfraction}{0.999999}
\renewcommand{\textfraction}{0.00001}
\renewcommand{\floatpagefraction}{0.9999999}


==> tab-previous-work.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{llllllll}
  \toprule
  &
  AML\cite{AcarBlDo07}
  &
  Sting\cite{AcarBlBlHaTa09}
  &
  DITTO\cite{ShankarBo07}
  &
  SAIL\cite{AcarAhBl08}
  &
  DeltaML\cite{Ley-WildFlAc08}
  &
  CEAL\cite{HammerAcCh09}
  &
  \textbf{SASM}
  \\

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
   \hline

  \textit{Memory Effects}
  &
  Write once
  &
  Write once
  &
  Pure
  &
  Imperative
  &
  Write once
  &
  Imperative
  &
  Imperative
  \\
  \hline

  \textit{Formal Semantics} &
  Yes & No & No & Yes & Yes & No & Yes
  \\
  
  \textit{\quad~Evaluation} &
  Big-step & -- & -- & Big-step & Big-step & -- & Small-step
  \\

  \textit{\quad~Control style}
  &
  Direct
  &
  --
  &
  --
  &
  Direct
  &
  Cont.-passing
  &
  --
  &
  Direct
  \\

  \textit{\quad~Trace reuse}
  &
  Oracular
  &
  --
  &
  --
  &
  Oracular
  &
  Edit-based
  &
  --
  &
  Edit-based
  \\

  \hline

  \textit{Implementation} &
  No & Yes & Yes & Yes & Yes & Yes & Yes
  \\
  \textit{\quad~Host language}
  &
  -- & SML & Java & SML & SML & C & C
  \\
  
  \textit{\quad~Host support}
  &
  -- & Lib & VM & Lib & Compiler & Compiler & Compiler

  \\
  \textit{\quad~Custom GC}
  &
  -- & No & No & No & No & Yes & Yes
  \\
  \bottomrule
\end{tabular}
\end{center}
\nocaptionrule
\caption{Comparison to previous work on self-adjusting computation}
\end{table*}

